Contrastive Alignment of Vision to Language Through Parameter-Efficient Transfer Learning

Contrastive vision-language models (e.g. CLIP) are typically created by updating all the parameters of a vision model and language model through contrastive training. Can such models be created by a small number of parameter updates to an already-trained language model and vision model? The literature describes techniques that can create vision-language models by updating a small number of parameters in a language model, but these require already aligned visual representations and are non-contrastive, hence unusable for latency-sensitive applications such as neural search. We explore the feasibility and benefits of parameter-efficient contrastive vision-language alignment through transfer learning: creating a model such as CLIP by minimally updating an already-trained vision and language model. We find that a minimal set of parameter updates ($<$7%) can achieve the same performance as full-model training, and updating specific components ($<$1% of parameters) can match 75% of full-model training. We describe a series of experiments: we show that existing knowledge is conserved more strongly in parameter-efficient training and that parameter-efficient scaling scales with model and dataset size. Where paired-image text data is scarce but strong multilingual language models exist (e.g. low resource languages), parameter-efficient training is even preferable to full-model training. Given a fixed compute budget, parameter-efficient training allows training larger models on the same hardware, achieving equivalent performance in less time. Parameter-efficient training hence constitutes an energy-efficient and effective training strategy for contrastive vision-language models that may be preferable to the full-model training paradigm for common use cases. Code and weights at https://github.com/codezakh/LilT.

==> figures/ablations.tex <==
\begin{table}[]
    \centering
        \caption{}
    \label{tab:ablations}
\begin{tabular}{lccccccccc}
% \hline & \multicolumn{4}{c}{ Pre-training Task } & & \multicolumn{2}{c}{ Zero-Shot Performance } \\
% \cline { 2 - 5 } \cline { 6 - 7 } 
\toprule
% \multicolumn{4}{c}{Components} &  \multicolumn{5}{c}{Flickr30k True 0-shot (1k test set)} \\
\multicolumn{4}{c}{Components} &  & \multicolumn{2}{c}{Flickr} & \multicolumn{2}{c}{COCO} & IN2 \\
\cmidrule(l{0.5em}r{0.5em}){2-4}  \cmidrule(l{0.5em}r{0.5em}){6-10}
& Projection & Unlocked LN & Adapter & \% Trained & TR & IR & TR & IR & Acc-1 \\
\midrule 
(a) & $\checkmark$ &  & & 0.04\% & 24.3 & 21.59 & 19.5 & 16.6 & 4.27 \\
(a) & & $\checkmark$ & & 0.20\% & 38.7 & 31.8 & 34.2 & 29.1 & 6.7 \\
(b) & $\checkmark$ & $\checkmark$  &  & 0.24\% & 62.3 & 51.7 & 56.8 & 47.2 & 12.45 \\
(c) & $\checkmark$ &  & $\checkmark$ & 6.96\% & 57.5 & 47.8 & 61.6 & 51.3 & 9.02 \\
(d) & $\checkmark$& $\checkmark$& $\checkmark$ & 6.99\% & 68.8 & 58.46 & 72.2 & 61.8 & 12.94  \\
% \midrule
% (d) &$\checkmark$ & $\checkmark$& $\checkmark$  & & 86.2 & 97.2 & 98.7 & 69.5 & 90.2 \\
% &  & Method &  & \%  & TR & IR & TR & IR & Acc-1 \\
% &  & Method &  &  &  & &  &  &  \\
% \midrule
% (d) &  \texttt{bert-base} & +Freeze ViT & (LiT) & 56.0 \% & 66.06 & 53.52 & 80.5 & 68.6 & 15.0  \\
% (d) & & CLIP &  & 100.0\% & 75.8 & 65.9 & 86.1 & 78.0 & 12.29  \\
\bottomrule
% (e) & $\checkmark$ & & $\checkmark$ & & & $-$ & $-$ & & & &\\
% (f) & $\checkmark$ & & & $\checkmark$ & & $-$ & $-$ & & & &\\
% (g) & & $\checkmark$ & $\checkmark$ & & & $-$ & $-$ & & & &\\
% \hline (h) & $\checkmark$ & & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% (i) & $\checkmark$ & $\checkmark$ & & $\checkmark$ & & $-$ & $-$ & & & &\\
% (j) & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & $-$ & $-$ & & & &\\
% (k) & & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% (k) & & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% \hline (l) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% \hline
\end{tabular}
\end{table}

==> figures/imagenet-a.tex <==
\begin{table}[]
    \centering
        \caption{
        Evaluation on additional zero-shot classification tasks. 
        \textbf{First place} is in bold and \textcolor{red}{second place} is in red. 
        \colorbox{LimeGreen}{LilT} models are boxed in green.
        Acc-1 stands for top-1 accuracy, and Acc-5 is top-5 accuracy.
        Higher is better.
        }
    \label{tab:additional-datasets}
\begin{tabular}{lccccc}
% \hline & \multicolumn{4}{c}{ Pre-training Task } & & \multicolumn{2}{c}{ Zero-Shot Performance } \\
% \cline { 2 - 5 } \cline { 6 - 7 } 
\toprule
% \multicolumn{4}{c}{Components} &  \multicolumn{5}{c}{Flickr30k True 0-shot (1k test set)} \\
\multicolumn{4}{c}{Model} &  \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{ImageNet-A} \\
\cmidrule(l{0.5em}r{0.5em}){2-4}  \cmidrule(l{0.5em}r{0.5em}){5-6} \cmidrule(l{0.5em}r{0.5em}){7-8} \cmidrule(l{0.5em}r{0.5em}){9-10}
& Configuration & \# Trainable & \% Trained &  Acc-1 & Acc-5 & Acc-1 & Acc-5 & Acc-1 & Acc-5 \\
\midrule
  \rowcolor{LimeGreen}(a) & LilT-tiny & 736.45 K & 7.37  & 2.77 & 9.15  \\
 (b) & LiT-tiny & 4.45 M & 44.57 & 3.39 & 11.03  \\
 \rowcolor{LimeGreen}(c) & LilT-small & 5.19 M & 10.28 & 4.79 & 13.8  \\
 (d) & CLIP-tiny & 9.99 M & 100.0  & 2.73 & 10.49  \\
 \rowcolor{LimeGreen}(e) & LilT-base & 14.65 M & 7.51  & 5.11 & 15.8  \\
 \rowcolor{LimeGreen}(f) & LilT-large & 25.92 M & 4.06  & \textbf{7.61} & \textbf{23.44}  \\
 (g) & LiT-small & 28.73 M & 56.98 & 26.88 & 47.17 & 12.3 & \textcolor{red}{59.17} & 5.37 & 16.01  \\
 (h) & CLIP-small & 50.42 M & 100.0 & 26.43 & 49.54 & 7.18 & 54.41 & 4.41 & 14.45  \\
 (i) & LiT-base & 109.28 M & 56.01 & 26.15 & 48.69 & 11.51 & 55.75 & \textcolor{red}{5.92} & \textcolor{red}{18.13}  \\
 (j) & CLIP-base & 195.13 M & 100.0 & 25.25 & 50.93 & 9.47 & 53.33 & 4.68 & 16.41  \\
%  \midrule
%  (k) & VGG-19 & 143M M & 100.0 & - & - & - & - & - & -  \\
\bottomrule
% (e) & $\checkmark$ & & $\checkmark$ & & & $-$ & $-$ & & & &\\
% (f) & $\checkmark$ & & & $\checkmark$ & & $-$ & $-$ & & & &\\
% (g) & & $\checkmark$ & $\checkmark$ & & & $-$ & $-$ & & & &\\
% \hline (h) & $\checkmark$ & & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% (i) & $\checkmark$ & $\checkmark$ & & $\checkmark$ & & $-$ & $-$ & & & &\\
% (j) & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & $-$ & $-$ & & & &\\
% (k) & & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% (k) & & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% \hline (l) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $-$ & $-$ & & & &\\
% \hline
\end{tabular}
\end{table}
